XC-Cache: Cross-Attending to Cached Context for Efficient LLM Inference

In-context learning (ICL) approaches typically leverage prompting to condition decoder-only language model generation on reference information. Just-in-time processing of a context is inefficient due to the quadratic cost of self-attention operations, and caching is desirable. However, caching transformer states can easily require almost as much space as the model parameters. When the right context isn't known in advance, caching ICL can be challenging. This work addresses these limitations by introducing models that, inspired by the encoder-decoder architecture, use cross-attention to condition generation on reference text without the prompt. More precisely, we leverage pre-trained decoder-only models and only train a small number of added layers. We use Question-Answering (QA) as a testbed to evaluate the ability of our models to perform conditional generation and observe that they outperform ICL, are comparable to fine-tuned prompted LLMs, and drastically reduce the space footprint relative to standard KV caching by two orders of magnitude.

==> arxiv-v1/table_all_results.tex <==
\renewcommand{\arraystretch}{1.25}
 \begin{table*}[th!]
 \centering
 \small
 \begin{tabular}{llccccccc}
 \toprule
Dataset & Model                     & EM & Precision & Recall & F1 & Rouge-L & METEOR &  \textsc{BERTScore}  \\
         \midrule
\multirow{8}{*}{Natural Questions} 
         & \textsc{GPT-3.5 Turbo}     & 43.08 & 55.10 & 74.87 & 57.80 & 57.67 & 53.22 & 90.87 \\
         & \textsc{FiD}               & 50.64 & 63.18 & 58.63 & 59.05 & 59.02 & 47.06 & 91.75 \\
         & \textsc{FiD} (fine-tuned)  & 67.00 & 75.20 & 72.59 & 72.67 & 72.52 & 58.30 & 94.76 \\
         & \llamachat{}               & 24.96 & 40.41 & 58.20 & 41.26 & 41.28 & 38.04 & 87.43 \\
         & \llama{} (LoRA)            & 59.64 & 70.55 & 67.39 & 67.38 & 67.08 & 53.88 & 93.27 \\
         \cmidrule(ll){2-9}
         & \ourmodelencoder{} (Ours)  & 56.77 & 65.93 & 62.89 & 63.12 & 62.99 & 49.99 & 93.30 \\
         & \ourmodel{} (Ours)         & 51.41 & 62.62 & 60.01 & 59.95 & 60.21 & 47.47 & 92.87 \\ 
 \midrule
 \multirow{8}{*}{HotpotQA} 
         & \textsc{GPT-3.5 Turbo}     & 27.62 & 39.08 & 46.43 & 39.37 & 39.35 & 34.01 & 87.83 \\
         & \textsc{FiD}               & 33.81 & 48.95 & 45.54 & 45.60 & 45.63 & 35.24 & 90.56 \\
         & \textsc{FiD} (fine-tuned)  & 44.04 & 54.49 & 55.38 & 53.54 & 53.42 & 41.78 & 89.64 \\
         & \llamachat{}               & 14.22 & 27.07 & 51.48 & 29.63 & 29.56 & 30.82 & 86.02 \\
         & \llama{} (LoRA)            & 58.33 & 74.91 & 72.72 & 71.97 & 71.91 & 55.27 & 94.62 \\
         \cmidrule(ll){2-9}
         & \ourmodelencoder{} (Ours)  & 43.29 & 56.88 & 54.90 & 54.57 & 54.63 & 41.13 & 92.08 \\
         & \ourmodel{} (Ours)         & 31.90 & 46.27 & 44.02 & 43.94 & 44.35 & 32.17 & 90.55 \\
 \midrule
 \multirow{8}{*}{TopiOCQA} 
         & \textsc{GPT-3.5 Turbo}     & 17.18 & 44.29 & 45.77 & 40.18 & 39.23 & 35.50 & 87.52 \\
         & \textsc{FiD}               & 16.43 & 53.56 & 27.17 & 31.22 & 31.02 & 20.56 & 85.95 \\
         & \textsc{FiD} (fine-tuned)  & 24.94 & 49.80 & 41.69 & 41.52 & 41.31 & 32.31 & 86.54 \\
         & \llamachat{}               & 13.76 & 42.56 & 36.87 & 33.45 & 32.88 & 26.95 & 86.33 \\
         & \llama{} (LoRA)            & 25.89 & 61.29 & 57.43 & 55.41 & 54.92 & 47.19 & 90.80 \\
         \cmidrule(ll){2-9}
         & \ourmodelencoder{} (Ours)  & 24.82 & 55.44 & 47.83 & 47.73 & 47.49 & 39.22 & 89.40 \\
         & \ourmodel{} (Ours)         & 19.17 & 52.49 & 46.64 & 45.47 & 44.94 & 38.37 & 89.16 \\
 \bottomrule
 \end{tabular}

 \caption{Question-Answer performance on three diverse information-seeking tasks. All models in this table that are trained/fine-tuned, did so on the same five datasets; the table reports the metrics of testing these models on different test splits.}

 \label{tab:correctness_main_results}
 \end{table*}



==> arxiv-v1/table_hotpot.tex <==
\renewcommand{\arraystretch}{1.25}
\begin{table}[th!]
 \centering
 \small
 \begin{tabular}{l|c|cccc}
 \toprule
       & \multicolumn{5}{|c}{Positions of the useful contexts} \\ \\
       &                       Shuffled & Beginning & Middle &  End & Far apart \\
 Model &                            &  0,1 & 4,5 & 8,9 & 0,9   \\
 \midrule
           \llamachat{}                &  \underline{29.63} &  \textbf{33.88} &  30.45 & 32.80 & 32.05 \\
           \llama{} (LoRA)             &  \underline{71.97} &  72.28 &  71.83 & \textbf{74.35} & 73.14 \\
           \ourmodel{} (Ours)          &  \underline{43.94} &  43.52 &  \textbf{44.30} & 42.30 & 43.70 \\
           \ourmodelencoder{} (Ours)   &  \underline{54.57} &  \textbf{57.65} &  56.79 & 54.61 & 52.98 \\
 \bottomrule
 \end{tabular}

 \caption{Results on HotpotQA when we vary the position of the two useful contexts (out of a total of roughly 10 contexts per sample). We test beginning (positions 0, 1), middle (positions 4, 5), end (positions 8, 9) positions, and the case where the two contexts are far apart (positions 0, 9).}


\label{tab:results_hotpot}
\end{table}

==> arxiv-v1/table_icl.tex <==
\setlength{\tabcolsep}{4pt}
\begin{table}[t!]
  \centering
  \small
  \resizebox{\columnwidth}{!}{
  \begin{tabular}{llcc}
\toprule
Dataset           & Model                     & \multicolumn{1}{l}{\textsc{F1}} & \multicolumn{1}{l}{\textsc{BERTScore}} \\ \midrule
                  & \textsc{GPT-3.5 Turbo}             & 57.80                           & 90.87                                  \\
                  & \textsc{FiD}                    & 59.05                           & 91.75                                  \\
                  \cmidrule(lr){2-4} 
\textsc{NQ}       & \llamachat{}              & 41.26                           & 87.43                                  \\
                  & \ourmodel{} (Ours)        & 59.95                           & 92.87                                  \\
                  & \ourmodelencoder{} (Ours) & \textbf{63.12}                  & \textbf{93.30}                         \\ \midrule
                  & \textsc{GPT-3.5 Turbo}             & 39.37                           & 87.83                                  \\
                  & \textsc{FiD}                    & 45.60                           & 90.56                                  \\ 
                  \cmidrule(lr){2-4} 
\textsc{HotpotQA} & \llamachat{}              & 29.63                           & 86.02                                  \\
                  & \ourmodel{} (Ours)        & 43.94                           & 90.55                                  \\
                  & \ourmodelencoder{} (Ours) & \textbf{54.57}                  & \textbf{92.08}                         \\ \midrule
                  & \textsc{GPT-3.5 Turbo}             & 40.18                           & 87.52                                  \\
                  & \textsc{FiD}                    & 31.22                           & 85.95                                  \\ 
                  \cmidrule(lr){2-4} 
\textsc{TopiOCQA} & \llamachat{}              & 33.45                           & 86.33                                  \\
                  & \ourmodel{} (Ours)        & 45.47                           & 89.16                                  \\
                  & \ourmodelencoder{} (Ours) & \textbf{47.73}                  & \textbf{89.40}                         \\ \bottomrule
\end{tabular}
}
  \caption{Question-Answer performance on three diverse information-seeking tasks. \textsc{GPT-3.5 Turbo} and \textsc{Llama2-Chat} are given reference context through ICL (prompting), while our approach uses cross-attention layers to ingest reference embeddings.}

  \label{tab:results_icl}
 \end{table}
 

==> arxiv-v1/table_lora.tex <==
\setlength{\tabcolsep}{4pt}
\begin{table}[t!]
 \centering
 \small
 \resizebox{\columnwidth}{!}{
 \begin{tabular}{llcc}
\toprule
Dataset           & Model                     & \textsc{F1}    & \textsc{BERTScore} \\ \midrule
                  & \textsc{GPT-3.5 Turbo}    & 57.80          & 90.87              \\
                  & \textsc{FiD} (fine-tuned) & \textbf{72.67} & \textbf{94.76}     \\ 
                  \cmidrule(lr){2-4}
\textsc{NQ}       & \llama{} (LoRA)           & 67.38          & 93.27              \\
                  & \ourmodel{} (Ours)        & 59.95          & 92.87              \\
                  & \ourmodelencoder{} (Ours) & 63.12          & 93.30              \\ \midrule
                  & \textsc{GPT-3.5 Turbo}    & 39.37          & 87.83              \\
                  & \textsc{FiD} (fine-tuned) & 53.54          & 89.64              \\ 
                  \cmidrule(lr){2-4} 
\textsc{HotpotQA} & \llama{} (LoRA)           & \textbf{71.97} & \textbf{94.62}     \\
                  & \ourmodel{} (Ours)        & 43.94          & 90.55              \\
                  & \ourmodelencoder{} (Ours) & 54.57          & 92.08              \\ \midrule
                  & \textsc{GPT-3.5 Turbo}    & 40.18          & 87.52              \\
                  & \textsc{FiD} (fine-tuned) & 41.52          & 86.54              \\ 
                  \cmidrule(lr){2-4}
\textsc{TopiOCQA} & \llama{} (LoRA)           & \textbf{55.41} & \textbf{90.80}     \\
                  & \ourmodel{} (Ours)        & 45.47          & 89.16              \\
                  & \ourmodelencoder{} (Ours) & 47.73          & 89.40              \\ \bottomrule
\end{tabular}}

 \caption{Question-Answer performance with ICL, carried out with a model specialized to a prompt template via \textsc{LoRA}. Note that the FiD model was pre-trained on \nq{}, hence its high performance on that dataset.}

 \label{tab:results_lora}
 \end{table}

